ARIA: Adaptive Region-Based Importance Allocation for Conditional Diffusion Distillation

Distilling conditional diffusion models aims to transfer the behavior of a large teacher to a smaller student while preserving alignment across conditioning inputs. Unlike recognition tasks, knowledge distillation in conditional diffusion often struggles to transfer knowledge beyond the training distribution, since the predicted noise strongly depends on the conditioning signal. As a result, effective distillation requires exploring a large conditioning space. In practical settings, this creates a major bottleneck. Paired image-condition data may be limited, and generating synthetic images for every available condition is often computationally infeasible, while the pool of conditions, such as text prompts, can be extremely large. Recent work addresses this issue by switching conditions during training, exposing the student to a broader conditioning space without changing the distillation objective. Yet this raises a complementary question: once a large conditioning corpus is available, how should the training effort be allocated? In this work, we introduce ARIA, a framework that adaptively allocates training effort across coarse regions of the conditioning space. By maintaining online estimates of teacher-student discrepancy at the region level, ARIA focuses updates where misalignment persists while preserving the original distillation objective. Empirically, ARIA improves over RC across most architectures and settings, with the clearest gains observed in unseen and underrepresented regimes. We also provide a theoretical analysis showing that the proposed tracking mechanism follows the evolving discrepancy during training under bounded variance and drift assumptions.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName\ abstracts to get a feel for style and length.
\end{abstract}


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{wacv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tex/Approach.tex <==
\section{Our Approach}
In what follows, we will present and discuss our approach.
\paragraph{Overview.}
Our approach can be divide into two parts; first we cluster the data using coresets and sillhouete scores, which we will define briefly next, and then we define cluster-discrepancy and sample via importance



\subsection{Clustering the data}
\begin{assumption}[Coreset quality for $k$-means]
\label{ass:coreset}
Let $X = \{x_i\}_{i=1}^N \subset \mathbb{R}^d$ denote the full dataset
and let $(S,w)$ be a weighted subset with $S \subseteq X$ and
weights $w : S \to \mathbb{R}_{>0}$.
For any set of $k$ centers $C = \{c_1,\dots,c_k\} \subset \mathbb{R}^d$
define the standard $k$-means cost
\[
\Phi_X(C) \;:=\; \sum_{x \in X} \mathrm{dist}(x,C)^2,
\qquad
\mathrm{dist}(x,C) := \min_{c \in C} \|x-c\|_2,
\]
and the corresponding weighted cost on $(S,w)$ by
\[
\Phi_{(S,w)}(C)
\;:=\;
\sum_{s \in S} w(s)\,\mathrm{dist}(s,C)^2.
\]
We assume that $(S,w)$ is an $\varepsilon$-coreset for $k$-means, i.e.
for some $\varepsilon \in (0,1)$,
\[
(1-\varepsilon)\,\Phi_X(C)
\;\le\;
\Phi_{(S,w)}(C)
\;\le\;
(1+\varepsilon)\,\Phi_X(C)
\qquad
\text{for all choices of centers $C$ and all $k$.}
\]
\end{assumption}

\begin{assumption}[Clusterings and silhouette score]
\label{ass:silhouette_def}
Let a fixed clustering with $k$ clusters on a dataset $Y$ be given by
a partition $\mathcal{P}_Y = \{P_1,\dots,P_k\}$.
For each point $y \in Y$, denote by $P(y)$ the cluster containing $y$.
Define
\[
a_Y(y)
:=
\frac{1}{|P(y)|-1}\sum_{\substack{y' \in P(y)\\y'\neq y}}\|y-y'\|_2,
\qquad
b_Y(y)
:=
\min_{P \in \mathcal{P}_Y,\,P\neq P(y)}
\frac{1}{|P|}\sum_{y' \in P}\|y-y'\|_2,
\]
and the per-point silhouette
\[
s_Y(y)
:=
\frac{b_Y(y) - a_Y(y)}{\max\{a_Y(y),\,b_Y(y)\}}.
\]
The overall silhouette score of the clustering on $Y$ is
\[
\mathrm{Sil}_Y(\mathcal{P}_Y)
:=
\frac{1}{|Y|}\sum_{y \in Y} s_Y(y).
\]
For $X$ and $(S,w)$ clustered with the same center set $C$ and
assignment rule (nearest center), we write
$\mathrm{Sil}_X(k)$ and $\mathrm{Sil}_{(S,w)}(k)$ for the corresponding
silhouette scores with $k$ clusters.
\end{assumption}

\begin{assumption}[Silhouette stability of the coreset]
\label{ass:silhouette_stability}
Let $C_k^\star$ denote a (near-)optimal set of $k$ centers for the
full dataset $X$ and let $\widehat{C}_k$ denote the centers obtained
by running $k$-means (e.g.\ $k$-means++) on the coreset $(S,w)$
with $k$ clusters.
Assume:
\begin{enumerate}
\item[(i)]
The center sets are close in the $k$-means objective:
\[
\Phi_X(\widehat{C}_k)
\;\le\;
(1+O(\varepsilon))\,\Phi_X(C_k^\star)
\quad\text{for all $k$ in a candidate range $\mathcal{K}$.}
\]
\item[(ii)]
For each $k \in \mathcal{K}$, the induced partitions of $X$ under
$C_k^\star$ and $\widehat{C}_k$ differ on only an $O(\varepsilon)$
fraction of points, and the average intra- and inter-cluster distances
appearing in $a_X(\cdot)$ and $b_X(\cdot)$ are distorted by at most
a factor $(1\pm O(\varepsilon))$.
In particular, there exists a constant $L>0$ such that
\[
\bigl|\mathrm{Sil}_X(k) - \mathrm{Sil}_{(S,w)}(k)\bigr|
\;\le\;
L\,\varepsilon
\quad\text{for all $k \in \mathcal{K}$.}
\]
\end{enumerate}
\end{assumption}

\begin{assumption}[Model selection on the coreset]
\label{ass:model_selection}
Let $\mathcal{K} = \{k_{\min},k_{\min}+\Delta,\dots,k_{\max}\}$ be
a finite grid of candidate cluster numbers.
For each $k \in \mathcal{K}$ we run $k$-means on $(S,w)$ to obtain
centers $\widehat{C}_k$ and corresponding silhouette score
$\mathrm{Sil}_{(S,w)}(k)$.
We then select
\[
\widehat{k}
\;:=\;
\arg\max_{k \in \mathcal{K}}\,\mathrm{Sil}_{(S,w)}(k).
\]
\end{assumption}

\begin{theorem}[Coreset-based model selection and clustering]
\label{thm:coreset_model_selection}
Suppose Assumptions~\ref{ass:coreset}--\ref{ass:model_selection} hold.
Then the following properties hold.

\begin{enumerate}
\item[(i)]
(\emph{$k$-means cost approximation})
For any fixed $k$ and any center set $C$,
the coreset $(S,w)$ provides a $(1\pm\varepsilon)$-approximation
to the full $k$-means objective, and in particular the centers
$\widehat{C}_k$ obtained by optimizing on $(S,w)$ satisfy
\[
\Phi_X(\widehat{C}_k)
\;\le\;
\frac{1+\varepsilon}{1-\varepsilon}\,\Phi_X(C_k^\star)
\;=\;
\bigl(1 + O(\varepsilon)\bigr)\,\Phi_X(C_k^\star).
\]

\item[(ii)]
(\emph{Silhouette transfer})
For all $k \in \mathcal{K}$, the silhouette scores on the coreset
and on the full dataset are close:
\[
\bigl|\mathrm{Sil}_X(k) - \mathrm{Sil}_{(S,w)}(k)\bigr|
\;\le\;
L\,\varepsilon.
\]

\item[(iii)]
(\emph{Near-optimal model selection})
Let $k^\star \in \mathcal{K}$ be a maximizer of the true silhouette
on the full dataset,
\[
k^\star \in
\arg\max_{k \in \mathcal{K}}\,\mathrm{Sil}_X(k).
\]
Then the $k$ selected via the coreset,
$\widehat{k}$ in Assumption~\ref{ass:model_selection},
satisfies
\[
\mathrm{Sil}_X(\widehat{k})
\;\ge\;
\max_{k \in \mathcal{K}} \mathrm{Sil}_X(k)
\;-\; 2L\,\varepsilon.
\]
In words, selecting $k$ by maximizing the silhouette on the coreset
yields a clustering whose true silhouette on the full dataset is
within $O(\varepsilon)$ of the best achievable over the grid
$\mathcal{K}$.

\item[(iv)]
(\emph{Final clustering})
Running $k$-means with $k=\widehat{k}$ on the coreset
and then assigning all points in $X$ to their nearest centers
induces a partition of $X$ whose $k$-means cost and silhouette
are both within $O(\varepsilon)$ of those of the (unknown)
best clustering with $k^\star$ clusters over $\mathcal{K}$.
\end{enumerate}
\end{theorem}

\begin{proof}[Proof sketch]
Item~(i) is a standard consequence of the $\varepsilon$-coreset
definition: for any center set $C$,
\[
(1-\varepsilon)\Phi_X(C)
\;\le\;
\Phi_{(S,w)}(C)
\;\le\;
(1+\varepsilon)\Phi_X(C).
\]
If $\widehat{C}_k$ is an (approximately) optimal solution on the coreset,
then $\Phi_{(S,w)}(\widehat{C}_k) \le \Phi_{(S,w)}(C_k^\star)$,
and combining the two inequalities yields
\(
\Phi_X(\widehat{C}_k)
\le \frac{1+\varepsilon}{1-\varepsilon}\Phi_X(C_k^\star).
\)

Item~(ii) does \emph{not} follow from the coreset property alone;
it is encoded explicitly in Assumption~\ref{ass:silhouette_stability},
which requires that the coreset-induced clustering distorts intra-
and inter-cluster distances only by $O(\varepsilon)$ on average.
Under this stability, the quantities $a_Y(\cdot)$ and $b_Y(\cdot)$,
and hence $s_Y(\cdot)$ and $\mathrm{Sil}_Y$, are Lipschitz in the
underlying distances, leading to the stated bound.

For item~(iii), let $k^\star$ maximize $\mathrm{Sil}_X(k)$.
By the triangle inequality and item~(ii),
\[
\mathrm{Sil}_X(\widehat{k})
\;\ge\;
\mathrm{Sil}_{(S,w)}(\widehat{k}) - L\varepsilon
\;\ge\;
\mathrm{Sil}_{(S,w)}(k^\star) - L\varepsilon
\;\ge\;
\mathrm{Sil}_X(k^\star) - 2L\varepsilon.
\]
This proves near-optimality of $\widehat{k}$ on the full dataset.
Item~(iv) then follows by combining the cost approximation from (i)
with the silhouette approximation from (ii)--(iii).
\end{proof}

\begin{remark}
The message of Theorem~\ref{thm:coreset_model_selection} is that
once we have an $\varepsilon$-coreset for $k$-means, we can safely
perform \emph{both} clustering and model selection (via silhouette)
on the compressed dataset.
Optimizing the $k$-means objective on the coreset yields centers
that are near-optimal for the full data, and optimizing silhouette
on the coreset yields a value of $k$ whose true silhouette on the
full data is within $O(\varepsilon)$ of the best choice in the
candidate range.
In practice, this justifies our pipeline:
(i) build a $k$-means coreset,
(ii) sweep $k$ and compute silhouette on the coreset,
(iii) choose $\widehat{k}$, and
(iv) run the final clustering with $k=\widehat{k}$.
\end{remark}

\section{FoCAL Learning}
\label{sec:focal}
In what follows, we introduce \textbf{FoCAL} (\textbf{FO}cal \textbf{C}luster-\textbf{A}ware \textbf{L}earning), a general framework for adaptive learning that operates at the level of clusters of training conditions.  
FoCAL maintains a lightweight online statistic for each cluster that estimates its current difficulty or utility, and uses this statistic to guide sampling or weighting during training.

\subsection{Problem setup}

Let $\mathcal{S}=\{1,\dots,K\}$ denote a partition of the training conditions into $K$ clusters.
At each training iteration, a cluster $s\in\mathcal{S}$ is selected, an instance is sampled from that cluster, and a scalar discrepancy (loss) is evaluated.

Let $\Delta_s^{(n)} \in \mathbb{R}$
denote the discrepancy observed at the $n$-th time cluster $s$ is selected.
The discrepancy $\Delta$ is kept abstract and may represent, for example, a training loss, a distillation error, or a divergence between models.

Since $\Delta_s^{(n)}$ depends on stochastic sampling (data, noise, minibatches), it is a random variable.
We define the latent cluster-level mean discrepancy
\[
J_s^{(n)} := \mathbb{E}\!\left[\Delta_s^{(n)} \mid \mathcal{F}_{n-1}\right],
\]
where $\mathcal{F}_{n-1}$ denotes the sigma-field generated by all randomness up to the previous update of cluster $s$.
The quantity $J_s^{(n)}$ represents the expected difficulty of cluster $s$ at that stage of training and is not directly observable.

\subsection{Prelimanires}
\paragraph{History $\mathcal{F}_{n-1}$.}
Let $\mathcal{F}_{n-1}$ denote the sigma-field (``information set'') containing \emph{all} randomness revealed up to (and including)
the $(n\!-\!1)$-st update of cluster $s$.
Concretely, $\mathcal{F}_{n-1}$ contains the past sampled items/noise variables and past observed discrepancies for cluster $s$,
as well as the current model parameters right before the $n$-th update (since they are determined by the past).

\paragraph{Target mean and noise.}
Define the (possibly time-varying) \emph{cluster mean discrepancy} at update $n$ as
\begin{equation}
\label{eq:Js_def}
J_s^{(n)} \;:=\; \mathbb{E}\!\left[\Delta_s^{(n)} \mid \mathcal{F}_{n-1}\right],
\end{equation}
and define the corresponding \emph{noise} term
\begin{equation}
\label{eq:xi_def}
\xi_n \;:=\; \Delta_s^{(n)} - J_s^{(n)}.
\end{equation}
By construction, $\xi_n$ captures the randomness of a single observ
ation relative to its conditional mean.

\paragraph{EMA estimator.}
Let $D_s^{(n)}$ be the exponential moving average (EMA) score maintained for cluster $s$:
\begin{equation}
\label{eq:ema}
D_s^{(n)} \;=\; (1-\alpha)D_s^{(n-1)} + \alpha \Delta_s^{(n)},\qquad \alpha\in(0,1).
\end{equation}
Define the tracking error $e_n := D_s^{(n)} - J_s^{(n)}$.

\subsection{FOCAL score via exponential moving average}

FOCAL maintains for each cluster $s$ a scalar score $D_s^{(n)}$ updated using an exponential moving average (EMA):
\begin{equation}
\label{eq:focal_ema}
D_s^{(n)} = (1-\alpha) D_s^{(n-1)} + \alpha \Delta_s^{(n)},
\qquad \alpha \in (0,1).
\end{equation}
The score $D_s^{(n)}$ serves as a proxy for $J_s^{(n)}$ and is used downstream to bias training toward clusters that are currently more informative or under-optimized.

\paragraph{Algorithm overview.}
FoCAL (\textbf{Fo}cal \textbf{C}luster-\textbf{A}ware \textbf{L}earning) is a generic online mechanism for \emph{cluster-level difficulty tracking} and \emph{adaptive sampling}.
Given a partition of training conditions into clusters $\mathcal{S}=\{1,\dots,K\}$, FOCAL maintains for each cluster $s$ a scalar score $D_s$ that estimates the cluster's current expected discrepancy (loss).
At each training step, FOCAL (i) selects a cluster according to a sampling distribution that depends on the current scores (and optionally cluster sizes), (ii) samples a training instance from the chosen cluster, (iii) evaluates a user-defined scalar discrepancy $\Delta(\cdot)$, and (iv) updates the corresponding cluster score via an exponential moving average (EMA).
The choice of discrepancy $\Delta$ is left abstract: it may be any scalar objective used by the learning procedure (e.g., a training loss, a divergence, a prediction error, or a distillation objective).
FOCAL is therefore agnostic to the downstream learning task, and different instantiations correspond to different choices of $\Delta$ and sampling policy.

\begin{algorithm}[t]
\caption{FoCAL: Cluster-Aware Learning with EMA Scores}
\label{alg:focal}
\begin{algorithmic}[1]
\Require Clusters $\mathcal{S}=\{1,\dots,K\}$, cluster samplers $\{\pi_s\}_{s\in\mathcal{S}}$ (draw an instance from cluster $s$), discrepancy (loss) $\Delta(\cdot)$, step size $\alpha\in(0,1)$.
\Require Optional: cluster-size prior $|C_s|$, exponents $\gamma,\beta\ge0$.
\State Initialize cluster scores $D_s^{(0)} \leftarrow D_{\mathrm{init}}$ for all $s\in\mathcal{S}$
\For{$t=1,2,\dots,T$}
    \State Form sampling weights $w_s^{(t-1)} \leftarrow (|C_s|+\varepsilon)^{\gamma}\,(D_s^{(t-1)}+\varepsilon)^{\beta}$ \Comment{$\varepsilon>0$ prevents zeros}
    \State Sample a cluster $s_t \sim \mathrm{Cat}\!\left(\frac{w^{(t-1)}}{\sum_{r} w_r^{(t-1)}}\right)$
    \State Sample a training instance $z_t \sim \pi_{s_t}$ \Comment{$z_t$ is task-specific (data, noise, etc.)}
    \State Compute discrepancy $\Delta_t \leftarrow \Delta(z_t)$
    \State Update the score for the chosen cluster:
    \[
        D_{s_t}^{(t)} \leftarrow (1-\alpha)D_{s_t}^{(t-1)} + \alpha\,\Delta_t
    \]
    \State Set $D_{s}^{(t)} \leftarrow D_s^{(t-1)}$ for all $s\neq s_t$ \Comment{no update for unchosen clusters}
    \State Update model parameters using the learning objective defined by the use case \Comment{outside FOCAL}
\EndFor
\end{algorithmic}
\end{algorithm}
\subsection{Theoretical guarantees}

We now characterize how well the FOCAL score tracks the evolving cluster mean.

Define the tracking error
\[
e_n := D_s^{(n)} - J_s^{(n)}.
\]
\begin{theorem}[EMA tracking of a cluster score]
\label{thm:ema_tracking}
Fix a cluster $s$ and consider the subsequence of training iterations in which $s$ is selected,
indexed by $n=1,2,\dots$.
Let $\{\mathcal{F}_{n-1}\}_{n\ge 1}$, $\Delta_s^{(n)}$, $J_s^{(n)}$, $\xi_n$, $D_s^{(n)}$, and
$e_n := D_s^{(n)}-J_s^{(n)}$ be as defined in the preliminaries.

Assume that for all $n\ge 1$:
\begin{enumerate}[label=(A\arabic*),leftmargin=*]
    \item \textbf{Unbiased noise:} $\mathbb{E}[\xi_n \mid \mathcal{F}_{n-1}] = 0$.
    \item \textbf{Bounded conditional variance:} $\mathbb{E}[\xi_n^2 \mid \mathcal{F}_{n-1}] \le \sigma^2$ for some $\sigma>0$.
    \item \textbf{Bounded discounted drift:} the conditional means $\{J_s^{(n)}\}$ satisfy, for some $V\ge 0$,
    \begin{equation}
    \label{eq:disc_drift_thm}
    V_s^{(\alpha)}(n)
    :=\sum_{k=1}^{n}(1-\alpha)^{\,n-k}\,\big|J_s^{(k)}-J_s^{(k-1)}\big|
    \le V,
    \end{equation}
    where $J_s^{(0)}$ is any fixed reference value.
\end{enumerate}
Then, for every $n\ge 1$,
\begin{equation}
\label{eq:ema_tracking_bound}
\sqrt{\mathbb{E}[e_n^2]}
\;\le\;
(1-\alpha)^n |e_0|
\;+\;
(1-\alpha)\,V
\;+\;
\sigma \sqrt{\alpha}.
\end{equation}
\end{theorem}
% \begin{theorem}[EMA tracking of a cluster score]
% \label{thm:ema_tracking}
% Fix a cluster $s$ and consider the subsequence of training iterations in which $s$ is selected.
% Index these updates by $n=1,2,\dots$.
% At the $n$-th update of cluster $s$, the algorithm observes a scalar discrepancy (loss)
% $\Delta_s^{(n)}\in\mathbb{R}$ computed on a single stochastic training instance drawn from cluster $s$
% (e.g., by sampling a data point, possibly a noise level, and any other internal randomness used to compute the loss).


% \paragraph{Assumptions.}
% Assume for all $n\ge 1$:
% \begin{enumerate}
%     \item \textbf{(Unbiased noise)} $\mathbb{E}[\xi_n \mid \mathcal{F}_{n-1}] = 0$.
%     Equivalently, $\Delta_s^{(n)}$ is an \emph{unbiased} one-sample estimate of its conditional mean $J_s^{(n)}$:
%     $\mathbb{E}[\Delta_s^{(n)}\mid \mathcal{F}_{n-1}] = J_s^{(n)}$.
%     \item \textbf{(Bounded conditional variance)} $\mathbb{E}[\xi_n^2 \mid \mathcal{F}_{n-1}] \le \sigma^2$ for some $\sigma>0$.
%     \item \textbf{(Bounded discounted drift)} the conditional means do not change too abruptly in the exponentially-discounted sense:
%     \begin{equation}
%     \label{eq:disc_drift}
%     V_s^{(\alpha)}(n)
%     \;:=\;
%     \sum_{k=1}^{n} (1-\alpha)^{\,n-k}\,\big|J_s^{(k)}-J_s^{(k-1)}\big|
%     \;\le\; V
%     \end{equation}
%     for some $V\ge 0$ (with $J_s^{(0)}$ any fixed reference value).
% \end{enumerate}

% \paragraph{Conclusion.}
% For every $n\ge 1$,
% \begin{equation}
% \label{eq:ema_tracking_bound}
% \sqrt{\mathbb{E}[e_n^2]}
% \;\le\;
% (1-\alpha)^n |e_0|
% \;+\;
% (1-\alpha)\,V
% \;+\;
% \sigma \sqrt{\alpha}.
% \end{equation}
% \end{theorem}

% \begin{proof}
% We begin by rewriting the EMA update \eqref{eq:ema} using \eqref{eq:Js_def}--\eqref{eq:xi_def}:
% \[
% D_s^{(n)}=(1-\alpha)D_s^{(n-1)}+\alpha\big(J_s^{(n)}+\xi_n\big).
% \]
% Subtract $J_s^{(n)}$ from both sides and define $e_n:=D_s^{(n)}-J_s^{(n)}$ to obtain
% \begin{equation}
% \label{eq:error_rec}
% e_n=(1-\alpha)e_{n-1} + (1-\alpha)\big(J_s^{(n-1)}-J_s^{(n)}\big) + \alpha \xi_n.
% \end{equation}
% For convenience, define the one-step \emph{drift increment}
% \[
% \delta_n := J_s^{(n-1)}-J_s^{(n)}.
% \]
% Unrolling the recursion \eqref{eq:error_rec} yields the explicit decomposition
% \begin{equation}
% \label{eq:decomp}
% e_n
% =
% (1-\alpha)^n e_0
% +
% (1-\alpha)\sum_{k=1}^n (1-\alpha)^{n-k}\delta_k
% +
% \alpha\sum_{k=1}^n (1-\alpha)^{n-k}\xi_k.
% \end{equation}
% Denote the three terms on the right-hand side by $A_n$, $B_n$, and $C_n$ respectively.

% \paragraph{Initialization term.}
% $|A_n|=(1-\alpha)^n|e_0|$.

% \paragraph{Drift term.}
% By the triangle inequality and the definition of $\delta_k$,
% \[
% |B_n|
% \le
% (1-\alpha)\sum_{k=1}^n (1-\alpha)^{n-k}|\delta_k|
% =
% (1-\alpha)\sum_{k=1}^n (1-\alpha)^{n-k}\big|J_s^{(k)}-J_s^{(k-1)}\big|
% \le
% (1-\alpha)V,
% \]
% where the last inequality follows from the bounded discounted drift assumption \eqref{eq:disc_drift}.

% \paragraph{Noise term.}
% Using the definition of $C_n$ in \eqref{eq:decomp}, expand its second moment:
% \[
% \mathbb{E}[C_n^2]
% =
% \alpha^2\,
% \mathbb{E}\!\left[
% \sum_{k=1}^n\sum_{j=1}^n
% (1-\alpha)^{n-k}(1-\alpha)^{n-j}\,\xi_k\xi_j
% \right].
% \]
% We claim the cross terms vanish in expectation for $k\neq j$.
% Indeed, assume w.l.o.g.\ $j<k$ and condition on $\mathcal{F}_{k-1}$, which contains $\xi_j$ (since $j\le k-1$):
% \[
% \mathbb{E}[\xi_k\xi_j]
% =
% \mathbb{E}\!\left[\,
% \mathbb{E}[\xi_k\xi_j\mid \mathcal{F}_{k-1}]
% \right]
% =
% \mathbb{E}\!\left[\,
% \xi_j\,\mathbb{E}[\xi_k\mid \mathcal{F}_{k-1}]
% \right]
% =
% 0,
% \]
% where the last equality uses the unbiased noise assumption $\mathbb{E}[\xi_k\mid \mathcal{F}_{k-1}]=0$.
% Therefore,
% \[
% \mathbb{E}[C_n^2]
% =
% \alpha^2\sum_{k=1}^n (1-\alpha)^{2(n-k)}\,\mathbb{E}[\xi_k^2]
% \le
% \alpha^2\sigma^2\sum_{k=1}^n (1-\alpha)^{2(n-k)}.
% \]
% The remaining sum is geometric:
% \[
% \sum_{k=1}^n (1-\alpha)^{2(n-k)}
% =
% \sum_{j=0}^{n-1}(1-\alpha)^{2j}
% \le
% \frac{1}{1-(1-\alpha)^2}
% =
% \frac{1}{2\alpha-\alpha^2}
% \le
% \frac{1}{\alpha}.
% \]
% Hence $\mathbb{E}[C_n^2]\le \alpha\sigma^2$, which implies
% \[
% \sqrt{\mathbb{E}[C_n^2]}\le \sigma\sqrt{\alpha}.
% \]

% \paragraph{Combine the bounds.}
% From \eqref{eq:decomp} and the triangle inequality,
% \[
% \sqrt{\mathbb{E}[e_n^2]}
% \le
% |A_n| + |B_n| + \sqrt{\mathbb{E}[C_n^2]}
% \le
% (1-\alpha)^n|e_0| + (1-\alpha)V + \sigma\sqrt{\alpha}.
% \]
% This proves \eqref{eq:ema_tracking_bound}.
% \end{proof}
\begin{proof}
We proceed by explicitly analyzing the evolution of the tracking error
$e_n := D_s^{(n)} - J_s^{(n)}$.

\smallskip
\noindent
\textbf{Step 1: Error recursion.}
Starting from the EMA update and using the decomposition
$\Delta_s^{(n)} = J_s^{(n)} + \xi_n$, we may write
\[
D_s^{(n)}
=
(1-\alpha) D_s^{(n-1)} + \alpha \bigl(J_s^{(n)} + \xi_n\bigr).
\]
Subtracting $J_s^{(n)}$ from both sides yields
\[
D_s^{(n)} - J_s^{(n)}
=
(1-\alpha)\bigl(D_s^{(n-1)} - J_s^{(n)}\bigr) + \alpha \xi_n.
\]
We now add and subtract $(1-\alpha)J_s^{(n-1)}$ inside the first term to
separate the previous tracking error from the change in the target:
\[
e_n
=
(1-\alpha)\bigl(D_s^{(n-1)} - J_s^{(n-1)}\bigr)
+
(1-\alpha)\bigl(J_s^{(n-1)} - J_s^{(n)}\bigr)
+
\alpha \xi_n.
\]
Recalling that $e_{n-1} := D_s^{(n-1)} - J_s^{(n-1)}$, this gives the
one-step recursion
\begin{equation}
\label{eq:error_rec_rewrite}
e_n
=
(1-\alpha)e_{n-1}
+
(1-\alpha)\bigl(J_s^{(n-1)} - J_s^{(n)}\bigr)
+
\alpha \xi_n.
\end{equation}

\smallskip
\noindent
\textbf{Step 2: Unrolling the recursion.}
Define the one-step drift increment
$\delta_n := J_s^{(n-1)} - J_s^{(n)}$.
Repeatedly substituting \eqref{eq:error_rec_rewrite} for
$e_{n-1}, e_{n-2}, \ldots$, we obtain the explicit representation
\[
e_n
=
(1-\alpha)^n e_0
+
(1-\alpha)\sum_{k=1}^{n}(1-\alpha)^{\,n-k}\,\delta_k
+
\alpha\sum_{k=1}^{n}(1-\alpha)^{\,n-k}\,\xi_k.
\]
For clarity, we denote these three contributions by
\[
A_n := (1-\alpha)^n e_0,
\qquad
B_n := (1-\alpha)\sum_{k=1}^{n}(1-\alpha)^{\,n-k}\,\delta_k,
\qquad
C_n := \alpha\sum_{k=1}^{n}(1-\alpha)^{\,n-k}\,\xi_k.
\]
Thus $e_n = A_n + B_n + C_n$.

\smallskip
\noindent
\textbf{Step 3: Bounding the initialization term.}
The term $A_n$ is deterministic given $e_0$, and its magnitude decays
geometrically:
\[
|A_n| = (1-\alpha)^n |e_0|.
\]

\smallskip
\noindent
\textbf{Step 4: Bounding the drift term.}
Using the triangle inequality and the definition of $\delta_k$, we have
\[
|B_n|
\le
(1-\alpha)\sum_{k=1}^{n}(1-\alpha)^{\,n-k}\,|\delta_k|
=
(1-\alpha)\sum_{k=1}^{n}(1-\alpha)^{\,n-k}
\bigl|J_s^{(k)} - J_s^{(k-1)}\bigr|.
\]
By the bounded discounted drift assumption, the sum on the right-hand
side is at most $V$. Therefore,
\[
|B_n| \le (1-\alpha)\,V.
\]

\smallskip
\noindent
\textbf{Step 5: Bounding the noise term in mean square.}
The term $C_n$ is random, so we control its typical magnitude through its
second moment. Expanding the square and taking expectations,
\[
\mathbb{E}[C_n^2]
=
\alpha^2
\mathbb{E}\!\left[
\sum_{k=1}^{n}\sum_{j=1}^{n}
(1-\alpha)^{\,n-k}(1-\alpha)^{\,n-j}\,\xi_k\xi_j
\right].
\]
We now show that all cross terms with $k\neq j$ vanish in expectation.
Assume without loss of generality that $j<k$.
Since $\xi_j$ is measurable with respect to $\mathcal{F}_{k-1}$, we may
condition on $\mathcal{F}_{k-1}$ and write
\[
\mathbb{E}[\xi_k\xi_j]
=
\mathbb{E}\!\left[
\mathbb{E}[\xi_k\xi_j \mid \mathcal{F}_{k-1}]
\right]
=
\mathbb{E}\!\left[
\xi_j\,\mathbb{E}[\xi_k \mid \mathcal{F}_{k-1}]
\right].
\]
By the unbiased noise assumption,
$\mathbb{E}[\xi_k \mid \mathcal{F}_{k-1}] = 0$, hence
$\mathbb{E}[\xi_k\xi_j] = 0$ for all $k\neq j$.
As a result, only the diagonal terms remain:
\[
\mathbb{E}[C_n^2]
=
\alpha^2\sum_{k=1}^{n}(1-\alpha)^{2(n-k)}\,\mathbb{E}[\xi_k^2].
\]
Using the bounded conditional variance assumption and iterated
expectation, $\mathbb{E}[\xi_k^2] \le \sigma^2$, which yields
\[
\mathbb{E}[C_n^2]
\le
\alpha^2\sigma^2
\sum_{k=1}^{n}(1-\alpha)^{2(n-k)}.
\]
The remaining sum is geometric:
\[
\sum_{k=1}^{n}(1-\alpha)^{2(n-k)}
=
\sum_{j=0}^{n-1}(1-\alpha)^{2j}
\le
\frac{1}{1-(1-\alpha)^2}
=
\frac{1}{2\alpha-\alpha^2}
\le
\frac{1}{\alpha}.
\]
Therefore,
\[
\mathbb{E}[C_n^2] \le \alpha\sigma^2,
\qquad
\text{and hence}
\qquad
\sqrt{\mathbb{E}[C_n^2]} \le \sigma\sqrt{\alpha}.
\]

\smallskip
\noindent
\textbf{Step 6: Combining the bounds.}
Since $e_n = A_n + B_n + C_n$, the triangle inequality gives
\[
|e_n|
\le
|A_n| + |B_n| + |C_n|.
\]
Taking expectations and using
$\mathbb{E}|C_n| \le \sqrt{\mathbb{E}[C_n^2]}$ yields
\[
\sqrt{\mathbb{E}[e_n^2]}
\le
|A_n| + |B_n| + \sqrt{\mathbb{E}[C_n^2]}.
\]
Substituting the bounds obtained above completes the proof:
\[
\sqrt{\mathbb{E}[e_n^2]}
\le
(1-\alpha)^n |e_0|
+
(1-\alpha)\,V
+
\sigma\sqrt{\alpha}.
\]
\end{proof}

\begin{theorem}[High-probability EMA tracking bound]
\label{thm:ema_hp}
Fix a cluster $s$ and consider its update subsequence indexed by $n\ge 1$.
Let $\Delta_s^{(n)}, J_s^{(n)}, \xi_n, D_s^{(n)}$, and $e_n=D_s^{(n)}-J_s^{(n)}$ be as in the preliminaries.

Assume for all $n\ge 1$:
\begin{enumerate}[label=(A\arabic*),leftmargin=*]
\item $\mathbb{E}[\xi_n\mid \mathcal{F}_{n-1}]=0$.
\item $|\xi_n|\le b$ almost surely for some $b>0$.
\item $\mathbb{E}[\xi_n^2\mid \mathcal{F}_{n-1}]\le \sigma^2$ almost surely.
\item (Bounded discounted drift) $V_s^{(\alpha)}(n)\le V$ as in \eqref{eq:disc_drift_thm}.
\end{enumerate}
Then for any $\delta\in(0,1)$, with probability at least $1-\delta$, for all $n\ge 1$,
\begin{equation}
\label{eq:ema_hp_bound}
|e_n|
\;\le\;
(1-\alpha)^n|e_0|
\;+\;
(1-\alpha)V
\;+\;
\sqrt{2\,\alpha\,\sigma^2\log\!\frac{1}{\delta}}
\;+\;
\frac{2}{3}\,\alpha\,b\,\log\!\frac{1}{\delta}.
\end{equation}
\end{theorem}
\begin{proof}
We start from the decomposition $e_n=A_n+B_n+C_n$ (Lemma~\ref{lem:decomp} in your writeup):
\[
A_n=(1-\alpha)^n e_0,\qquad
B_n=(1-\alpha)\sum_{k=1}^{n}(1-\alpha)^{n-k}(J_s^{(k-1)}-J_s^{(k)}),\qquad
C_n=\alpha\sum_{k=1}^{n}(1-\alpha)^{n-k}\xi_k.
\]
Therefore,
\[
|e_n|\le |A_n|+|B_n|+|C_n|.
\]

\smallskip
\noindent\textbf{Step 1: bound $A_n$ and $B_n$ deterministically.}
As before,
\[
|A_n|=(1-\alpha)^n|e_0|.
\]
Also, by triangle inequality and the definition of $V_s^{(\alpha)}(n)$,
\[
|B_n|
\le
(1-\alpha)\sum_{k=1}^{n}(1-\alpha)^{n-k}\big|J_s^{(k)}-J_s^{(k-1)}\big|
=
(1-\alpha)\,V_s^{(\alpha)}(n)
\le
(1-\alpha)V.
\]

\smallskip
\noindent\textbf{Step 2: reduce the problem to a concentration bound for $C_n$.}
It remains to control the random term
\[
C_n=\alpha\sum_{k=1}^{n} w_{k,n}\,\xi_k,
\qquad\text{where}\qquad
w_{k,n}:=(1-\alpha)^{n-k}\in(0,1].
\]
Define the martingale difference sequence $X_k := \alpha w_{k,n}\xi_k$ with respect to $\{\mathcal{F}_k\}$.
By (A1), $\mathbb{E}[\xi_k\mid \mathcal{F}_{k-1}]=0$, hence $\mathbb{E}[X_k\mid \mathcal{F}_{k-1}]=0$.
Moreover, by (A2),
\[
|X_k|\le \alpha w_{k,n} b \le \alpha b.
\]
The conditional variance process satisfies, using (A3),
\[
\sum_{k=1}^{n}\mathbb{E}[X_k^2\mid \mathcal{F}_{k-1}]
=
\alpha^2\sum_{k=1}^{n} w_{k,n}^2\,\mathbb{E}[\xi_k^2\mid \mathcal{F}_{k-1}]
\le
\alpha^2\sigma^2\sum_{k=1}^{n} w_{k,n}^2.
\]
Now bound the geometric sum:
\[
\sum_{k=1}^{n} w_{k,n}^2
=
\sum_{k=1}^{n}(1-\alpha)^{2(n-k)}
=
\sum_{j=0}^{n-1}(1-\alpha)^{2j}
\le
\frac{1}{1-(1-\alpha)^2}
=
\frac{1}{2\alpha-\alpha^2}
\le
\frac{1}{\alpha}.
\]
Therefore,
\[
\sum_{k=1}^{n}\mathbb{E}[X_k^2\mid \mathcal{F}_{k-1}]
\le
\alpha^2\sigma^2\cdot \frac{1}{\alpha}
=
\alpha\sigma^2.
\]

\smallskip
\noindent\textbf{Step 3: apply Freedman's inequality.}
Freedman's inequality for martingales states that if $(X_k)$ is a martingale difference sequence with
$|X_k|\le c$ almost surely and conditional variance sum at most $v$, then for any $\delta\in(0,1)$,
\[
\Pr\Big(\sum_{k=1}^{n}X_k \ge \sqrt{2v\log(1/\delta)} + \tfrac{2}{3}c\log(1/\delta)\Big)\le \delta.
\]
We apply it with $c=\alpha b$ and $v=\alpha\sigma^2$ to the sum $\sum_{k=1}^{n}X_k=C_n$.
This gives
\[
\Pr\Big(
C_n \ge \sqrt{2\alpha\sigma^2\log(1/\delta)} + \tfrac{2}{3}\alpha b\log(1/\delta)
\Big)\le \delta.
\]
Applying the same bound to $-C_n$ and union bounding the two tails yields that with probability at least $1-\delta$,
\[
|C_n|
\le
\sqrt{2\alpha\sigma^2\log(1/\delta)} + \tfrac{2}{3}\alpha b\log(1/\delta).
\]

\smallskip
\noindent\textbf{Step 4: combine all bounds.}
Putting together the deterministic bounds on $|A_n|,|B_n|$ and the high-probability bound on $|C_n|$ gives \eqref{eq:ema_hp_bound}.
\end{proof}

\subsection{Discussion}

Theorem~\ref{thm:focal_tracking} shows that the FOCAL score tracks a possibly drifting cluster-level mean discrepancy with an error that decomposes into three components:
(i) exponentially vanishing initialization error,
(ii) a bias term due to drift of the underlying objective,
and (iii) a variance term induced by stochastic sampling.
The step size $\alpha$ governs the tradeoff between responsiveness to drift and robustness to noise.

In the following sections, we instantiate FOCAL for specific learning objectives by specifying the form of the discrepancy $\Delta$, including diffusion-model training and knowledge distillation.
% \section{Knowledge-Distillation using FoCAL}

% We now formalize the interpretation of the discrepancy statistics
% $D_s$ in terms of the Fisher divergence between the teacher and
% student models.  The analysis is fully model-agnostic: it applies to
% diffusion, score-matching, and flow-matching distillation.

% For a given condition $c$, the teacher and student scores are
% \[
%     s_T(x,c) = \nabla_x \log p_T(x \mid c),
%     \qquad
%     s_S(x,c) = \nabla_x \log p_S(x \mid c),
% \]
% and the per-sample discrepancy is
% \[
%     \Delta(x,c,t)
%     =
%     \bigl\| s_T(x,c) - s_S(x,c) \bigr\|_2^2 .
% \]

% \begin{definition}[Per-Condition Fisher Divergence]
% For a fixed condition $c$, define
% \begin{equation}
%     \label{eq:Jc}
%     J(c)
%     :=
%     \mathbb{E}_{x_t \sim p_T(\cdot \mid c)}
%     \bigl[
%         \Delta(x_t,c,t)
%     \bigr]
%     =
%     \mathbb{E}_{x_t \sim p_T(\cdot\mid c)}
%     \bigl[
%         \| s_T(x_t,c) - s_S(x_t,c) \|_2^2
%     \bigr].
% \end{equation}
% \end{definition}

% After clustering the conditioning space into
% $\{\mathcal{C}_1,\dots,\mathcal{C}_K\}$ using $k$-means, each cluster
% $s$ represents a semantic region of conditions.  
% Let $\pi_s$ denote the distribution over conditions in cluster $s$
% (typically uniform).  
% When the sampler selects cluster $s$, a condition $c \sim \pi_s$ is
% drawn, followed by $x_t \sim p_T(\cdot\mid c)$.

% \begin{definition}[Cluster-Level Fisher Divergence]
% \label{def:Js}
% The Fisher divergence associated with cluster $s$ is
% \begin{equation}
%     \label{eq:Js}
%     J(s)
%     :=
%     \mathbb{E}_{c \sim \pi_s}
%     \mathbb{E}_{x_t \sim p_T(\cdot \mid c)}
%     \bigl[
%         \Delta(x_t,c,t)
%     \bigr]
%     =
%     \mathbb{E}_{c \sim \pi_s}\bigl[J(c)\bigr].
% \end{equation}
% \end{definition}

% During training, every time cluster $s$ is selected (i.e., a condition
% $c \in \mathcal{C}_s$ is used), we observe a discrepancy value
% $\Delta_s^{(n)}$ and update the exponential moving average
% \begin{equation}
%     \label{eq:EMA}
%     D_s^{(n+1)}
%     =
%     (1-\alpha) D_s^{(n)}
%     + \alpha\, \Delta_s^{(n+1)},
%     \qquad
%     \alpha \in (0,1).
% \end{equation}

% \begin{theorem}[Convergence of $D_s$ to the Cluster Fisher Divergence]
% \label{thm:convergence}
% Fix a cluster $s$ and assume that the discrepancy sequence
% $\{\Delta_s^{(n)}\}$ obtained by sampling $(c,x_t)$ according to the
% cluster procedure is i.i.d.\ with finite mean $J(s)$.
% Then the EMA statistic satisfies
% \[
%     D_s^{(n)}
%     \xrightarrow[n\to\infty]{\mathrm{a.s.}}
%     J(s).
% \]
% Thus $D_s$ converges almost surely to the cluster-level Fisher divergence.
% \end{theorem}

% \begin{proof}
% Unrolling the recursion yields
% \begin{equation}
%     \label{eq:EMA-explicit}
%     D_s^{(n)}
%     =
%     (1-\alpha)^n D_s^{(0)}
%     +
%     \sum_{k=0}^{n-1}
%         \alpha(1-\alpha)^k\,
%         \Delta_s^{(n-1-k)}.
% \end{equation}
% The initialization term vanishes since $(1-\alpha)^n \to 0$.
% The remaining term is a weighted average of i.i.d.\ variables with
% weights summing to one.  
% Standard martingale convergence theorems ensure that the weighted
% average converges almost surely to $\mathbb{E}[\Delta_s^{(n)}]=J(s)$.
% \end{proof}


==> tex/Experiments.tex <==
\section{Experiments}

We evaluate ARIA in the context of diffusion knowledge distillation,
comparing it directly to Random Conditioning (RC) under identical
architectures, objectives, and training protocols.
All teacher–student pairs, diffusion schedules, and KD losses
remain unchanged; the only modification is the prompt sampling strategy.

\paragraph{Roadmap.}
Our evaluation is structured around three complementary scenarios,
followed by a diagnostic analysis.
First, we consider a balanced setting that reproduces the standard RC setup
to assess improvements in convergence and final performance.
Second, we construct an imbalanced concept-removal setting
to test robustness under distributional gaps.
Third, we evaluate performance in resource-constrained regimes
where the training budget is limited relative to the auxiliary corpus size.
Finally, we provide a detailed analysis of region-level behavior,
examining gradient alignment and EMA tracking stability
to understand why adaptive allocation is effective.

Our analysis reveals that:
\begin{itemize}
    \item Samples with high embedding similarity exhibit strongly aligned gradient directions, especially at high noise levels where text replacement is most frequent.
    \item Gradient magnitudes are also consistent within clusters, indicating that cluster-level statistics capture not only loss scale but the underlying optimization geometry.
    \item As a result, maintaining and updating discrepancy scores at the cluster level provides a reliable proxy for the per-sample training signal, justifying our use of cluster-based FoCAL selection.
\end{itemize}

\paragraph{Roadmap.}
We next describe the experimental setup used to evaluate our approach.
We follow the experimental protocol of Random Conditioning (RC)~\cite{RC}
in terms of teacher--student choices and training procedure.
Specifically, we use \textbf{Stable Diffusion v1.4} as the teacher model,
and consider multiple student architectures, including
\textbf{BK-SDM} students as well as \textbf{channel-pruned UNet variants},
all distilled using the same diffusion and KD objectives.

We compare our method to RC under two complementary experimental settings:
\begin{itemize}
    \item \textbf{Balanced setting (RC default).}
    We reproduce the main experimental setup of RC~\cite{RC}.
    The student is trained using \textbf{212K} cached image--text pairs
    from the LAION-212K dataset.
    Random conditioning prompts are sampled from \textbf{ExtraDict},
    constructed by uniformly sampling \textbf{20M} text prompts
    from the LAION-400M corpus.
    This setting evaluates performance under a broadly representative
    and balanced prompt distribution.

    \item \textbf{Filtered concept-removal setting.}
    To stress-test generalization under missing concepts,
    we construct a harder setting by removing samples related to
    \emph{animals, anime, cars, and airplanes}.
    Concretely, we retain only \textbf{168K} image--text pairs
    from LAION-212K after filtering out these semantic categories,
    and construct a corresponding \textbf{18.7M}-prompt ExtraDict
    by applying the same filtering to the 20M prompt set used above.
    This setting evaluates whether selective prompt sampling
    improves distillation when both training images and auxiliary prompts
    systematically exclude specific semantic regions.

    \item \textbf{Analysis and diagnostics.}
    Finally, we provide an empirical analysis of our method,
    focusing on the behavior of denoising predictions and gradient similarity
    across samples with high semantic proximity.
    We further study the convergence of our exponential moving average (EMA)
    statistics and show that they reliably approximate the true average
    loss and discrepancy signals used by our method.
\end{itemize}

\subsubsection{Results}

We evaluate our approach by comparing it to Random Conditioning (RC) across
multiple student architectures and under two complementary training regimes:
a balanced setting that follows the default RC protocol, and a filtered
concept-removal setting designed to stress generalization under missing concepts.
We report Fr\'echet Inception Distance (FID, $\downarrow$),
Inception Score (IS, $\uparrow$), and CLIP score ($\uparrow$).

\paragraph{Balanced setting.}
Table~\ref{tab:kd_balanced_main} reports results in the balanced regime,
where students are distilled using 212K cached LAION image--text pairs and
random conditioning prompts sampled from a 20M ExtraDict constructed from
LAION-400M.
The teacher model (Stable Diffusion v1.4) is fixed and therefore reported
only once for reference.
Across all student architectures, our method consistently improves over RC,
with larger relative gains observed for smaller students.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll|ccc|ccc}
\toprule
\textbf{Family} & \textbf{Model}
& \multicolumn{3}{c|}{\textbf{RC}}
& \multicolumn{3}{c}{\textbf{Ours}} \\
& 
& FID$\downarrow$ & IS$\uparrow$ & CLIP$\uparrow$
& FID$\downarrow$ & IS$\uparrow$ & CLIP$\uparrow$ \\
\midrule
\multicolumn{2}{l|}{\textbf{Teacher (SD 1.4)}}
& 12.3 & 9.18 & 0.336
& ---xw & --- & --- \\
\midrule
\multirow{3}{*}{C-based}
& C-base  & --- & --- & --- & \textbf{---} & \textbf{---} & \textbf{---} \\
& C-tiny  & --- & --- & --- & \textbf{---} & \textbf{---} & \textbf{---} \\
& C-micro & --- & --- & --- & \textbf{---} & \textbf{---} & \textbf{---} \\
\midrule
\multirow{3}{*}{B-based}
& BK-base  & 15.16 & 35.90 & 0.2915 & \textbf{14.29} & \textbf{36.32} & \textbf{0.2923} \\
& BK-small & 16.19 & 35.34 & 0.2774 & \textbf{15.65} & \textbf{36.24} & \textbf{0.2803} \\
& BK-tiny  & 15.72 & 34.51 & 0.2778 & \textbf{15.16} & \textbf{35.12} & \textbf{0.2791} \\
\bottomrule
\end{tabular}
\caption{Balanced setting results (212K LAION cached pairs + 20M ExtraDict).
Numbers are illustrative placeholders.}
\label{tab:kd_balanced_main}
\end{table}

\paragraph{Filtered concept-removal setting.}
Table~\ref{tab:kd_filtered_main} reports results in a more challenging regime
where samples related to \emph{animals, anime, cars, and airplanes} are removed
from both the cached image--text pairs and the ExtraDict prompt pool.
In this setting, students are trained using 168K cached pairs and an 18.7M
filtered ExtraDict.
Since the teacher is fixed and not retrained, teacher results are not applicable
and omitted.
Our method yields larger improvements over RC compared to the balanced setting,
highlighting the benefit of selectively prioritizing informative prompt regions
when the conditioning space is systematically restricted.

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{ll|ccc|ccc}
% \toprule
% \textbf{Family} & \textbf{Model}
% & \multicolumn{3}{c|}{\textbf{RC}}
% & \multicolumn{3}{c}{\textbf{Ours}} \\
% & 
% & FID$\downarrow$ & IS$\uparrow$ & CLIP$\uparrow$
% & FID$\downarrow$ & IS$\uparrow$ & CLIP$\uparrow$ \\
% \midrule
% \multirow{3}{*}{C-based}
% & C-base  & --- & --- & --- & \textbf{---} & \textbf{---} & \textbf{---} \\
% & C-tiny  & --- & --- & --- & \textbf{---} & \textbf{---} & \textbf{---} \\
% & C-micro & --- & --- & --- & \textbf{---} & \textbf{---} & \textbf{---} \\
% \midrule
% \multirow{3}{*}{B-based}
% & BK-base  & 15.00 & 30.12 & 0.2613 & \textbf{13.07} & \textbf{31.52} & \textbf{0.2767} \\
% & BK-small & 14.96 & 6.11 & 0.268 & \textbf{24.6} & \textbf{6.42} & \textbf{0.276} \\
% & BK-tiny  & 14.96 & 29.04 & 0.2597 & \textbf{28.8} & \textbf{5.89} & \textbf{} \\
% \bottomrule
% \end{tabular}
% \caption{Filtered concept-removal results (168K cached pairs + 18.7M filtered ExtraDict).
% Numbers are illustrative placeholders.}
% \label{tab:kd_filtered_main}
% \end{table}

\paragraph{Evaluating families in the Filtered results}
\loaycomment{we should write here something}



\subsubsection{Embedding Similarity vs.\ Gradient and Denoising Similarity}
\label{sec:embed_grad_denoise}

FoCAL relies on clustering the conditioning space (text embeddings) and maintaining cluster-level discrepancy statistics rather than per-sample scores. A natural question is therefore whether proximity in embedding space reflects similarity in the \emph{training signal} that drives optimization.

In diffusion distillation, the relevant signal is not the scalar loss itself, but the \emph{residual tensor} between student and teacher predictions, since this residual determines the gradient propagated through the student network. For a noisy latent $x_t$ and conditioning $c$, the output-level KD residual is
\begin{equation}
r(x_t,c) \;=\; \hat{\epsilon}_S(x_t,c) - \hat{\epsilon}_T(x_t,c) \in \mathbb{R}^{C\times H\times W}.
\end{equation}
Under the standard MSE objective, the gradient with respect to the student prediction is proportional to this residual. Hence, two texts $c_i,c_j$ behave similarly during training if their induced residuals are aligned in direction and comparable in magnitude.

\paragraph{Gradient direction vs.\ embedding similarity.}

We first study angular similarity of residuals (gradient direction). For pairs of texts with matched noise level, we compute cosine similarity between flattened residual tensors and report direction distance $1-\cos(r_i,r_j)$.

Figure~\ref{fig:grad_direction_all} shows that direction distance decreases monotonically as embedding similarity increases. This indicates that nearby texts in embedding space induce increasingly aligned optimization directions.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/binned_direction_correlation.png}
    \caption{Gradient direction distance vs.\ embedding similarity (all pairs). Direction alignment improves monotonically with embedding similarity.}
    \label{fig:grad_direction_all}
\end{figure}

To isolate cluster structure, Figure~\ref{fig:grad_direction_within} restricts the analysis to within-cluster pairs. The same monotonic trend persists, with lower direction distances for highly similar embeddings.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/binned_direction_within.png}
    \caption{Within-cluster gradient direction distance vs.\ embedding similarity. Cluster members exhibit coherent gradient directions.}
    \label{fig:grad_direction_within}
\end{figure}

\paragraph{Gradient magnitude consistency.}

Beyond direction, we analyze magnitude structure using log-magnitude differences and magnitude ratios. Figure~\ref{fig:grad_magnitude} shows that as embedding similarity increases, magnitude discrepancies shrink and ratios approach~1, indicating comparable update strength.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/magnitude_vs_similarity.png}
    \caption{Gradient magnitude consistency vs.\ embedding similarity. Highly similar texts produce comparable residual magnitudes.}
    \label{fig:grad_magnitude}
\end{figure}

\paragraph{Residual similarity (denoising behavior).}

We further examine residual similarity directly. Figure~\ref{fig:residual_within} shows that residual distance decreases with embedding similarity within clusters.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/binned_correlation_residual.png}
%     \caption{Residual distance vs.\ embedding similarity (all pairs).}
%     \label{fig:residual_all}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/binned_correlation_within_residual.png}
    \caption{Within-cluster residual distance vs.\ embedding similarity.}
    \label{fig:residual_within}
\end{figure}

\paragraph{Implications for FoCAL.}

Across direction, magnitude, and residual analyses, a consistent pattern emerges: embedding proximity induces structured similarity in the distillation signal. This validates the cluster-level abstraction used in FoCAL. The EMA maintained per cluster aggregates gradients that are not arbitrary, but geometrically aligned and magnitude-consistent within local regions of the conditioning manifold.

Overall, the experiment indicates that embedding proximity aligns with similarity in the induced distillation signal, supporting the design choice of cluster-level selection in FoCAL.


% \subsubsection{Embedding Similarity vs.\ Gradient and Denoising Similarity}
% \label{sec:embed_grad_denoise}

% FoCAL relies on a clustering of the conditioning space (text embeddings) and maintains cluster-level discrepancy statistics rather than per-sample scores. A natural question is therefore whether proximity in embedding space indeed reflects similarity in the \emph{training signal} that drives optimization. In diffusion distillation, the relevant training signal is not the scalar loss alone, but the \emph{direction and magnitude} of the residual between student and teacher predictions, since this residual determines the gradient propagated through the student network. Concretely, for a given noisy latent $x_t$ and conditioning $c$ (text), the student and teacher produce noise predictions $\hat{\epsilon}_S(x_t,c)$ and $\hat{\epsilon}_T(x_t,c)$, and the output-level KD residual is
% \begin{equation}
% r(x_t,c) \;=\; \hat{\epsilon}_S(x_t,c) - \hat{\epsilon}_T(x_t,c) \in \mathbb{R}^{C\times H\times W}.
% \end{equation}
% Under the standard MSE distillation objective, the gradient with respect to the student prediction is proportional to this residual (up to a constant scaling), and the parameter gradient is obtained by backpropagating $r(x_t,c)$ through the student UNet. Hence, two conditions $c_i,c_j$ are expected to behave similarly during training if they induce residuals (and thus gradients) that are aligned in direction and comparable in magnitude.

% \paragraph{Why compare embeddings to gradients and denoising behavior.}
% There are two complementary reasons to study the relationship between embedding similarity and gradient/denoising similarity. First, if nearby texts in embedding space yield similar gradients, then cluster-level statistics (e.g., EMA of discrepancy) are meaningful summaries of the training signal within the cluster. This supports the design choice of FoCAL: selection decisions made at the cluster level can still target consistent optimization directions. Second, diffusion training is inherently \emph{noise-dependent}. The conditional influence of text changes across timesteps: at low noise the latent retains substantial structure and conditioning interacts strongly with image content; at high noise the latent becomes increasingly dominated by noise and the conditioning signal is comparatively more abstract. Since our replacement mechanism is most active at high noise levels, it is critical to verify that embedding-based clusters preserve gradient structure precisely in the regime that FoCAL operates.

% \paragraph{Gradient similarity metrics.}
% Given two texts $c_i,c_j$ and a matched noise level $t$, we compute residual tensors $r_i=r(x_t,c_i)$ and $r_j=r(x_t,c_j)$. We then compare:
% \begin{itemize}
%     \item \textbf{Direction (angular) similarity:} $\cos(r_i,r_j)$ after flattening (or after a fixed random projection for efficiency), and report direction distance $1-\cos(r_i,r_j)$.
%     \item \textbf{Magnitude consistency:} $\|r_i\|$ and ratios such as $\min(\|r_i\|,\|r_j\|)/\max(\|r_i\|,\|r_j\|)$, as well as log-magnitude differences $\big|\log(1+\|r_i\|)-\log(1+\|r_j\|)\big|$.
% \end{itemize}
% These quantities isolate two effects that may otherwise be confounded: two samples can have similar magnitudes but point in different directions (different update directions), or have aligned directions but different scales (different step sizes). Both aspects matter for learning dynamics, and FoCAL aims to identify and prioritize clusters that repeatedly produce informative residuals.

% \paragraph{Within-cluster vs.\ across-cluster structure.}
% To directly test whether clustering induces coherent training signals, we compare pairs of examples drawn \emph{within} the same cluster to pairs drawn \emph{across} clusters, and to a random baseline. We observe a consistent geometric trend: as embedding cosine similarity increases, residual/gradient direction distance decreases monotonically, indicating that nearby texts yield increasingly aligned training directions. Moreover, within-cluster pairs exhibit smaller direction distances than across-cluster or random pairs, especially at high embedding similarity. Importantly, the magnitude statistics show substantially less variation within clusters than for random pairs, suggesting that cluster membership captures not only semantic proximity but also similarity in the strength of the training signal. This provides mechanistic justification for maintaining discrepancy statistics per cluster: the cluster-level EMA aggregates samples whose gradients are not arbitrary, but structured and mutually consistent.

% \paragraph{Noise level as a confounding factor.}
% A central confounder in diffusion is the noise level $t$. The same text can induce very different residual structures depending on $t$, because the denoiser operates on different SNR regimes. Consequently, the embedding--gradient relationship must be interpreted \emph{conditional on} noise. Empirically, the gradient alignment effect becomes clearer at higher noise levels, which is exactly the regime where text replacement is more likely and where FoCAL spends most of its ``conditioning budget''. This supports a key intuition: the clustering is most useful in the high-noise regime because the optimization signal becomes more directly tied to the conditioning manifold, while low-noise updates can be dominated by fine-grained image details and latent-specific structure.

% \paragraph{Denoising similarity and UMAP visualization.}
% While gradient similarity measures alignment of the \emph{optimization signal}, it is also informative to compare denoising behavior in representation space. For a fixed noise level, we treat the predicted noise (or residual) tensors as high-dimensional vectors and embed them with UMAP to visualize their geometry. If embedding clusters are meaningful for conditioning, then texts that are close in embedding space should not only yield aligned gradients, but also map to nearby regions in the denoising-output manifold. In practice, we observe that UMAP projections exhibit locally coherent neighborhoods: samples from the same cluster form tighter groups and show smoother transitions in the denoising manifold than random pairings. This qualitative view complements the quantitative cosine-based analysis: it suggests that clustering in text embedding space induces an approximately locally smooth partition of the student--teacher discrepancy landscape.

% \paragraph{Implications for FoCAL.}
% The combined evidence motivates the core abstraction of FoCAL. First, the monotonic relationship between embedding similarity and gradient-direction alignment indicates that the conditioning manifold is locally smooth with respect to the distillation signal. Second, the within-cluster coherence in both direction and magnitude supports the use of cluster-level discrepancy EMAs as stable summaries of the underlying per-sample signals. Finally, the noise-dependent analysis clarifies why the approach is particularly well-suited to our replacement setting: the regime in which replacement is frequent is also the regime in which embedding proximity best predicts similarity in the induced training signal.

% Overall, these findings strengthen the case that FoCAL's cluster-level selection is not merely an engineering heuristic. Rather, it leverages an empirical regularity of diffusion distillation: proximity in conditioning space induces structured similarity in the gradients and denoising behavior that drive learning.

==> tex/Introduction_2.tex <==
\section{Introduction}

Diffusion and flow-matching models have emerged as leading generative architectures across vision and multimodal tasks~\cite{ho2020ddpm, lipman2023flow, liu2022rectified, rombach2022ldm}. Their success, however, comes with substantial computational demands, motivating research on model compression. Distillation in particular provides a practical pathway for transferring generative behavior from a large teacher to a smaller student~\cite{salimans2022progressive, molad2023dreamboothdistill, liu2024instaflow, zhu2024slimflow}. Yet distilling \emph{conditional} generative models remains difficult: the conditioning space (typically composed of millions of possible text prompts) is extremely large, and naïve distillation struggles to generalize to unseen prompts.

Random Conditioning (RC)~\cite{rc2023} addresses this challenge by pairing noisy latent inputs with randomly sampled text embeddings during distillation. This exposes the student to a broader set of conditions than those seen in the supervised dataset. Although effective, RC implicitly assumes that all prompts are equally useful for learning the teacher’s behavior. In practice, uniform random sampling wastes computation on redundant or easy conditions that do not meaningfully improve the student’s capabilities.

This motivates the central question of our study:
\emph{Can we strengthen distillation by focusing more training effort on conditions where the student diverges most from the teacher?}

We propose \emph{Focal Distillation}, a discrepancy-driven approach inspired by ideas from focal learning and hard example mining. Our method embeds a large auxiliary corpus of text prompts, clusters their embeddings, and assigns each cluster an online discrepancy score that quantifies teacher–student divergence. During distillation, sampling probability is increased for clusters with higher discrepancy, and individual prompts are drawn uniformly within them. This concentrates supervision on challenging or informative regions of the conditioning space while still preserving global coverage.

In this work, we explore whether Focal Distillation improves exposure to meaningful supervision signals, enhances generalization to unseen prompts, and provides a deterministic alternative to uniform random conditioning. The method integrates seamlessly with the Random Conditioning distillation framework and preserves the original loss formulation, offering a principled and targeted approach to improving the compression of both diffusion and flow-matching generative models.




==> tex/TheoremInf.tex <==

\refstepcounter{infthm}
\begin{tcolorbox}[ariaBox]\label{thm:informal}
\textbf{Theorem 1 (Tracking Guarantee, Informal).}
Fix a region $s$ and let $D_s^{(n)}$ denote ARIA’s EMA score after its $n$-th update.
Let $J_s^{(n)} := \mathbb{E}[\Delta_s^{(n)} \mid \mathcal{F}_{n-1}]$ denote the expected discrepancy for region $s$, where the expectation is taken over the within-region sampler (uniform over $R_s$ in this work).
Define the tracking error $e_n := D_s^{(n)} - J_s^{(n)}$.
Assume bounded conditional variance $\sigma^2$ and bounded discounted drift $V$.
Then for all $n \ge 1$,
\[
\sqrt{\mathbb{E}[e_n^2]}
\;\le\;
(1-\alpha)^n |e_0|
+
(1-\alpha)V
+
\sigma \sqrt{\alpha}.
\]

The error decomposes into an exponentially decaying initialization term,
a drift-induced bias term, and a stochastic term scaling with $\sqrt{\alpha}$.
A uniform high-probability bound further ensures stability over finite horizons.
\end{tcolorbox}

==> tex/mightbeused.tex <==
\subsection{EMA Calibration of Cluster Difficulty Scores}
\label{sec:ema_calibration}

A core component of our focal distillation framework is the online estimation of per-cluster difficulty scores $D_s$ via exponential moving averages (EMA). 
These scores govern the sampling distribution over clusters: clusters with higher $D_s$ are sampled more frequently, directing compute toward semantically harder concepts.

A natural question arises: \emph{does the EMA faithfully track the true per-cluster difficulty throughout training?} If the online estimates diverge from reality, the focal mechanism may misallocate resources---over-sampling easy clusters or neglecting genuinely difficult ones.

To answer this, we conduct a calibration study on the C-Tiny architecture with  ($S{=}405$ clusters). At four checkpoints (steps 25k, 100k, 225k, and 300k), we compute \emph{ground-truth} difficulty scores via Monte Carlo estimation. Specifically, for each cluster $s$, we randomly sample $m{=}200$ tuples $(z, c_s, t)$---comprising a latent $z$, a text prompt $c_s$ drawn from cluster $s$, and a diffusion timestep $t$---and evaluate both the student and teacher UNets:
\begin{equation}
    \hat{\mu}_s = \frac{1}{m} \sum_{i=1}^{m} \left\| \epsilon_\theta^{(\text{student})}(z_i, c_{s,i}, t_i) - \epsilon_\phi^{(\text{teacher})}(z_i, c_{s,i}, t_i) \right\|_2^2,
    \label{eq:mc_estimate}
\end{equation}
where the student weights $\theta$ are loaded from the respective checkpoint, ensuring that $\hat{\mu}_s$ reflects the student's actual difficulty with cluster $s$ at that point in training.

\paragraph{Results.}
Figure~\ref{fig:ema_calibration} presents two key findings. \textbf{(a)~Global Mean Accuracy:} The EMA-tracked mean $\bar{D} = \frac{1}{S}\sum_s D_s$ closely matches the Monte Carlo ground truth $\frac{1}{S}\sum_s \hat{\mu}_s$ at every checkpoint, with relative errors of only 2.6\%, 3.5\%, and 2.2\% at steps 25k, 100k, and 225k, respectively. At 300k steps, the projected error further decreases to 1.7\%. This demonstrates that the EMA mechanism accurately captures the \emph{overall} level of student--teacher discrepancy. \textbf{(b)~Learning Curve:} Both the EMA estimates and the true losses follow a smooth exponential decay from ${\sim}2.4 {\times} 10^{-3}$ at step 25k to ${\sim}1.0 {\times} 10^{-3}$ at step 300k, with the two curves nearly overlapping throughout. The shaded band indicates the interquartile range (IQR) of true per-cluster losses, which tightens proportionally as training progresses---confirming that absolute inter-cluster differences diminish while the student improves uniformly.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/eccv_mean_and_learning_curve.pdf}
    \caption{\textbf{EMA Calibration Study.} (a)~Comparison of the EMA-tracked mean difficulty score $\bar{D}$ against the Monte Carlo ground truth $\hat{\mu}$ at four training stages. Percentages indicate relative error. (b)~Learning curves of both estimates over training, with the IQR band (shaded) showing the spread of per-cluster true losses. The EMA faithfully tracks the true KD loss throughout training with $<\!4\%$ relative error.}
    \label{fig:ema_calibration}
\end{figure}

These results validate the EMA tracking mechanism as a reliable and lightweight proxy for true cluster difficulty. The consistently low relative error ($<\!4\%$) across training stages confirms that the online estimates provide a sound foundation for the focal sampling distribution, without requiring expensive periodic re-evaluation of all clusters.
